Long term planning of military aircraft flight and maintenance operations

We present the Flight and Maintenance Planning (FMP) problem in its military variant and applied to long term planning. The problem has been previously studied for short- and medium-term horizons only. We compare its similarities and differences with previous work and prove its complexity. We generate scenarios inspired by the French Air Force fleet. We formulate an exact Mixed Integer Programming (MIP) model to solve the problem in these scenarios and we analyse the performance of the solving method under these circumstances. A heuristic was built to generate fast feasible solutions, that in some cases were shown to help warm-start the model.

==> gantts/gantt_complex.tex <==
\definecolor{color1}{HTML}{FFFFCC}
\definecolor{color2}{HTML}{FFEDA0}
\definecolor{color3}{HTML}{FED976}
\definecolor{color4}{HTML}{FEB24C}
\definecolor{color5}{HTML}{FD8D3C}
\definecolor{color6}{HTML}{FC4E2A}
\definecolor{color7}{HTML}{E31A1C}
\definecolor{color8}{HTML}{B10026}
\newcommand\Dganttbar[5]{
      \ganttbar[#5]{#1}{#3}{#4}\ganttbar[inline,bar label font=\tiny\color{white}\bfseries, #5]{#2}{#3}{#4}
    }
    \begin{ganttchart}[
    x unit=1cm,
    y unit chart=0.6cm,
    hgrid,
    vgrid,
    time slot format=isodate,
    time slot unit=month
    ]{2017-10-01}{2018-07-01}
    \gantttitlecalendar{year} \\
\Dganttbar{1}{A}{2017-11-01}{2018-01-01}{bar/.append style={fill=color1}}
\Dganttbar{1}{B}{2017-10-01}{2018-03-01}{bar/.append style={fill=color2}}\ganttnewline
\Dganttbar{2}{C}{2017-12-01}{2018-02-01}{bar/.append style={fill=color3}}\ganttnewline
\Dganttbar{3}{D}{2018-02-01}{2018-07-01}{bar/.append style={fill=color4}}\ganttnewline
\Dganttbar{4}{E}{2018-02-01}{2018-04-01}{bar/.append style={fill=color5}}\ganttnewline
\Dganttbar{5}{F}{2017-10-01}{2017-12-01}{bar/.append style={fill=color6}}\ganttnewline
\Dganttbar{6}{G}{2017-10-01}{2018-03-01}{bar/.append style={fill=color7}}\ganttnewline
\Dganttbar{7}{H}{2017-12-01}{2018-02-01}{bar/.append style={fill=color8}}
\end{ganttchart}


==> gantts/gantt_example.tex <==
\definecolor{color1}{HTML}{1A9641}
\definecolor{color2}{HTML}{D3D3D3}
\definecolor{color3}{HTML}{FDAE61}
\definecolor{color4}{HTML}{D7191C}
\definecolor{color5}{HTML}{A6D96A}
\newcommand\Dganttbar[5]{
      \ganttbar[#5]{#1}{#3}{#4}\ganttbar[inline,bar label font=\tiny\color{white}\bfseries, #5]{#2}{#3}{#4}
    }
    \begin{ganttchart}[
    expand chart=\textwidth,
y unit chart=0.5cm,
    hgrid,
    vgrid,
    time slot format=isodate-yearmonth,
    time slot unit=month
    ]{2018-01}{2025-06}
    \gantttitlecalendar{year} \\
\Dganttbar{0}{39h}{2018-01}{2018-04}{bar/.append style={fill=color1}}
\Dganttbar{0}{M}{2018-05}{2018-11}{bar/.append style={fill=color2}}
\Dganttbar{0}{48h}{2019-03}{2019-11}{bar/.append style={fill=color3}}
\Dganttbar{0}{31h}{2020-11}{2021-10}{bar/.append style={fill=color1}}
\Dganttbar{0}{M}{2023-03}{2023-09}{bar/.append style={fill=color2}}
\Dganttbar{0}{52h}{2023-10}{2024-04}{bar/.append style={fill=color3}}
\Dganttbar{0}{62h}{2024-04}{2025-03}{bar/.append style={fill=color4}}\ganttnewline
\Dganttbar{1}{39h}{2018-01}{2018-08}{bar/.append style={fill=color1}}
\Dganttbar{1}{M}{2019-01}{2019-07}{bar/.append style={fill=color2}}
\Dganttbar{1}{60h}{2023-01}{2023-10}{bar/.append style={fill=color4}}
\Dganttbar{1}{52h}{2023-10}{2024-04}{bar/.append style={fill=color3}}
\Dganttbar{1}{M}{2024-04}{2024-10}{bar/.append style={fill=color2}}\ganttnewline
\Dganttbar{2}{69h}{2018-08}{2019-03}{bar/.append style={fill=color4}}
\Dganttbar{2}{M}{2020-02}{2020-08}{bar/.append style={fill=color2}}
\Dganttbar{2}{60h}{2023-01}{2023-10}{bar/.append style={fill=color4}}\ganttnewline
\Dganttbar{3}{47h}{2019-11}{2020-08}{bar/.append style={fill=color3}}
\Dganttbar{3}{31h}{2020-11}{2021-10}{bar/.append style={fill=color1}}
\Dganttbar{3}{M}{2021-10}{2022-04}{bar/.append style={fill=color2}}\ganttnewline
\Dganttbar{4}{47h}{2020-07}{2020-11}{bar/.append style={fill=color3}}
\Dganttbar{4}{31h}{2020-11}{2021-10}{bar/.append style={fill=color1}}
\Dganttbar{4}{45h}{2021-10}{2022-05}{bar/.append style={fill=color5}}
\Dganttbar{4}{M}{2022-07}{2023-01}{bar/.append style={fill=color2}}\ganttnewline
\Dganttbar{5}{M}{2018-01}{2018-04}{bar/.append style={fill=color2}}
\Dganttbar{5}{39h}{2018-04}{2018-08}{bar/.append style={fill=color1}}
\Dganttbar{5}{47h}{2019-11}{2020-11}{bar/.append style={fill=color3}}
\Dganttbar{5}{M}{2022-12}{2023-06}{bar/.append style={fill=color2}}
\Dganttbar{5}{41h}{2025-03}{2025-06}{bar/.append style={fill=color5}}\ganttnewline
\Dganttbar{6}{69h}{2018-08}{2019-03}{bar/.append style={fill=color4}}
\Dganttbar{6}{45h}{2021-10}{2022-05}{bar/.append style={fill=color5}}
\Dganttbar{6}{M}{2022-05}{2022-11}{bar/.append style={fill=color2}}
\Dganttbar{6}{45h}{2022-11}{2023-01}{bar/.append style={fill=color5}}
\Dganttbar{6}{62h}{2024-04}{2025-03}{bar/.append style={fill=color4}}\ganttnewline
\Dganttbar{7}{M}{2018-02}{2018-08}{bar/.append style={fill=color2}}
\Dganttbar{7}{69h}{2018-08}{2019-03}{bar/.append style={fill=color4}}
\Dganttbar{7}{45h}{2021-10}{2022-05}{bar/.append style={fill=color5}}
\Dganttbar{7}{M}{2023-06}{2023-12}{bar/.append style={fill=color2}}
\Dganttbar{7}{62h}{2024-04}{2025-03}{bar/.append style={fill=color4}}\ganttnewline
\Dganttbar{8}{39h}{2018-01}{2018-08}{bar/.append style={fill=color1}}
\Dganttbar{8}{M}{2019-06}{2019-12}{bar/.append style={fill=color2}}
\Dganttbar{8}{31h}{2020-11}{2021-10}{bar/.append style={fill=color1}}
\Dganttbar{8}{60h}{2023-01}{2023-10}{bar/.append style={fill=color4}}
\Dganttbar{8}{M}{2023-11}{2024-05}{bar/.append style={fill=color2}}\ganttnewline
\Dganttbar{9}{47h}{2019-11}{2020-11}{bar/.append style={fill=color3}}
\Dganttbar{9}{M}{2021-03}{2021-09}{bar/.append style={fill=color2}}
\Dganttbar{9}{45h}{2022-05}{2023-01}{bar/.append style={fill=color5}}
\Dganttbar{9}{41h}{2025-03}{2025-06}{bar/.append style={fill=color5}}\ganttnewline
\Dganttbar{10}{39h}{2018-05}{2018-08}{bar/.append style={fill=color1}}
\Dganttbar{10}{69h}{2018-08}{2019-03}{bar/.append style={fill=color4}}
\Dganttbar{10}{M}{2020-06}{2020-12}{bar/.append style={fill=color2}}
\Dganttbar{10}{45h}{2022-05}{2023-01}{bar/.append style={fill=color5}}
\Dganttbar{10}{60h}{2023-01}{2023-10}{bar/.append style={fill=color4}}\ganttnewline
\Dganttbar{11}{M}{2018-08}{2019-02}{bar/.append style={fill=color2}}
\Dganttbar{11}{47h}{2019-11}{2020-11}{bar/.append style={fill=color3}}
\Dganttbar{11}{31h}{2020-11}{2021-10}{bar/.append style={fill=color1}}
\Dganttbar{11}{M}{2021-10}{2022-04}{bar/.append style={fill=color2}}
\Dganttbar{11}{45h}{2022-05}{2022-11}{bar/.append style={fill=color5}}
\Dganttbar{11}{62h}{2024-04}{2025-03}{bar/.append style={fill=color4}}\ganttnewline
\Dganttbar{12}{M}{2018-08}{2019-02}{bar/.append style={fill=color2}}
\Dganttbar{12}{48h}{2019-03}{2019-11}{bar/.append style={fill=color3}}
\Dganttbar{12}{47h}{2019-11}{2020-11}{bar/.append style={fill=color3}}
\Dganttbar{12}{M}{2022-11}{2023-05}{bar/.append style={fill=color2}}
\Dganttbar{12}{62h}{2024-04}{2025-03}{bar/.append style={fill=color4}}\ganttnewline
\Dganttbar{13}{45h}{2021-10}{2022-05}{bar/.append style={fill=color5}}
\Dganttbar{13}{M}{2022-05}{2022-11}{bar/.append style={fill=color2}}
\Dganttbar{13}{60h}{2023-01}{2023-10}{bar/.append style={fill=color4}}\ganttnewline
\Dganttbar{14}{39h}{2018-01}{2018-05}{bar/.append style={fill=color1}}
\Dganttbar{14}{48h}{2019-03}{2019-11}{bar/.append style={fill=color3}}
\Dganttbar{14}{M}{2020-10}{2021-04}{bar/.append style={fill=color2}}
\Dganttbar{14}{45h}{2021-10}{2022-05}{bar/.append style={fill=color5}}
\Dganttbar{14}{52h}{2023-10}{2024-04}{bar/.append style={fill=color3}}
\end{ganttchart}


==> gantts/gantt_heur1.tex <==
\definecolor{color1}{HTML}{1A9641}
\definecolor{color2}{HTML}{D3D3D3}
\definecolor{color3}{HTML}{FDAE61}
\definecolor{color4}{HTML}{D7191C}
\definecolor{color5}{HTML}{A6D96A}
\newcommand\Dganttbar[5]{
      \ganttbar[#5]{#1}{#3}{#4}\ganttbar[inline,bar label font=\tiny\color{white}\bfseries, #5]{#2}{#3}{#4}
    }
    \begin{ganttchart}[
    expand chart=\textwidth,
y unit chart=0.5cm,
    hgrid,
    vgrid,
    time slot format=isodate-yearmonth,
    time slot unit=month
    ]{2018-01}{2025-06}
    \gantttitlecalendar{year} \\
\Dganttbar{0}{39h}{2018-01}{2018-04}{bar/.append style={fill=color1}}
\Dganttbar{0}{M}{2018-05}{2018-11}{bar/.append style={fill=color2}}
\Dganttbar{0}{48h}{2019-03}{2019-11}{bar/.append style={fill=color3}}
\Dganttbar{0}{31h}{2020-11}{2021-10}{bar/.append style={fill=color1}}
\Dganttbar{0}{M}{2023-03}{2023-09}{bar/.append style={fill=color2}}
\Dganttbar{0}{52h}{2023-10}{2024-04}{bar/.append style={fill=color3}}
\Dganttbar{0}{62h}{2024-04}{2025-03}{bar/.append style={fill=color4}}\ganttnewline
\Dganttbar{1}{39h}{2018-01}{2018-08}{bar/.append style={fill=color1}}
\Dganttbar{1}{M}{2019-01}{2019-07}{bar/.append style={fill=color2}}
\Dganttbar{1}{60h}{2023-01}{2023-10}{bar/.append style={fill=color4}}
\Dganttbar{1}{52h}{2023-10}{2024-04}{bar/.append style={fill=color3}}
\Dganttbar{1}{M}{2024-04}{2024-10}{bar/.append style={fill=color2}}\ganttnewline
\Dganttbar{2}{69h}{2018-08}{2019-03}{bar/.append style={fill=color4}}
\Dganttbar{2}{M}{2020-02}{2020-08}{bar/.append style={fill=color2}}
\Dganttbar{2}{60h}{2023-01}{2023-10}{bar/.append style={fill=color4}}\ganttnewline
\Dganttbar{3}{47h}{2019-11}{2020-08}{bar/.append style={fill=color3}}
\Dganttbar{3}{31h}{2020-11}{2021-10}{bar/.append style={fill=color1}}
\Dganttbar{3}{M}{2021-10}{2022-04}{bar/.append style={fill=color2}}\ganttnewline
\Dganttbar{4}{47h}{2020-07}{2020-11}{bar/.append style={fill=color3}}
\Dganttbar{4}{31h}{2020-11}{2021-10}{bar/.append style={fill=color1}}
\Dganttbar{4}{45h}{2021-10}{2022-05}{bar/.append style={fill=color5}}
\Dganttbar{4}{M}{2022-07}{2023-01}{bar/.append style={fill=color2}}\ganttnewline
\Dganttbar{5}{M}{2018-01}{2018-04}{bar/.append style={fill=color2}}
\Dganttbar{5}{39h}{2018-04}{2018-08}{bar/.append style={fill=color1}}
\Dganttbar{5}{47h}{2019-11}{2020-11}{bar/.append style={fill=color3}}
\Dganttbar{5}{M}{2022-12}{2023-06}{bar/.append style={fill=color2}}
\Dganttbar{5}{41h}{2025-03}{2025-06}{bar/.append style={fill=color5}}\ganttnewline
\Dganttbar{6}{48h}{2019-03}{2019-11}{bar/.append style={fill=color3}}
\Dganttbar{6}{47h}{2019-11}{2020-11}{bar/.append style={fill=color3}}
\Dganttbar{6}{M}{2022-11}{2023-05}{bar/.append style={fill=color2}}
\Dganttbar{6}{62h}{2024-04}{2025-03}{bar/.append style={fill=color4}}\ganttnewline
\Dganttbar{7}{45h}{2021-10}{2022-05}{bar/.append style={fill=color5}}
\Dganttbar{7}{M}{2022-05}{2022-11}{bar/.append style={fill=color2}}
\Dganttbar{7}{60h}{2023-01}{2023-10}{bar/.append style={fill=color4}}\ganttnewline
\end{ganttchart}


==> gantts/gantt_heur2.tex <==
\definecolor{color1}{HTML}{1A9641}
\definecolor{color2}{HTML}{D3D3D3}
\definecolor{color3}{HTML}{FDAE61}
\definecolor{color4}{HTML}{D7191C}
\definecolor{color5}{HTML}{A6D96A}
\newcommand\Dganttbar[5]{
      \ganttbar[#5]{#1}{#3}{#4}\ganttbar[inline,bar label font=\tiny\color{white}\bfseries, #5]{#2}{#3}{#4}
    }
    \begin{ganttchart}[
    expand chart=\textwidth,
y unit chart=0.5cm,
    hgrid,
    vgrid,
    time slot format=isodate-yearmonth,
    time slot unit=month
    ]{2018-01}{2025-06}
    \gantttitlecalendar{year} \\
\Dganttbar{0}{39h}{2018-01}{2018-04}{bar/.append style={fill=color1}}
\Dganttbar{0}{M}{2018-05}{2018-11}{bar/.append style={fill=color2}}
\Dganttbar{0}{48h}{2019-03}{2019-11}{bar/.append style={fill=color3}}
\Dganttbar{0}{31h}{2020-11}{2021-10}{bar/.append style={fill=color1}}
\Dganttbar{0}{M}{2023-03}{2023-09}{bar/.append style={fill=color2}}
\Dganttbar{0}{52h}{2023-10}{2024-04}{bar/.append style={fill=color3}}
\Dganttbar{0}{62h}{2024-04}{2025-03}{bar/.append style={fill=color4}}\ganttnewline
\Dganttbar{1}{39h}{2018-01}{2018-08}{bar/.append style={fill=color1}}
\Dganttbar{1}{M}{2019-01}{2019-07}{bar/.append style={fill=color2}}
\Dganttbar{1}{60h}{2023-01}{2023-10}{bar/.append style={fill=color4}}
\Dganttbar{1}{52h}{2023-10}{2024-04}{bar/.append style={fill=color3}}
\Dganttbar{1}{M}{2024-04}{2024-10}{bar/.append style={fill=color2}}\ganttnewline
\Dganttbar{2}{69h}{2018-08}{2019-03}{bar/.append style={fill=color4}}
\Dganttbar{2}{M}{2020-02}{2020-08}{bar/.append style={fill=color2}}
\Dganttbar{2}{60h}{2023-01}{2023-10}{bar/.append style={fill=color4}}\ganttnewline
\Dganttbar{3}{47h}{2019-11}{2020-08}{bar/.append style={fill=color3}}
\Dganttbar{3}{31h}{2020-11}{2021-10}{bar/.append style={fill=color1}}
\Dganttbar{3}{M}{2021-10}{2022-04}{bar/.append style={fill=color2}}\ganttnewline
\Dganttbar{4}{47h}{2020-07}{2020-11}{bar/.append style={fill=color3}}
\Dganttbar{4}{45h}{2021-10}{2021-12}{bar/.append style={fill=color5}}
\Dganttbar{4}{31h}{2020-11}{2021-10}{bar/.append style={fill=color1}}\ganttnewline
\Dganttbar{5}{M}{2018-01}{2018-04}{bar/.append style={fill=color2}}\ganttnewline
\Dganttbar{6}{48h}{2019-03}{2019-11}{bar/.append style={fill=color3}}
\Dganttbar{6}{47h}{2019-11}{2020-11}{bar/.append style={fill=color3}}
\Dganttbar{6}{62h}{2024-04}{2025-03}{bar/.append style={fill=color4}}\ganttnewline
\Dganttbar{7}{45h}{2021-10}{2021-12}{bar/.append style={fill=color5}}
\Dganttbar{7}{60h}{2023-01}{2023-10}{bar/.append style={fill=color4}}\ganttnewline
\end{ganttchart}


==> gantts/time_windows.tex <==
% Same month implies one month
% so i need to take one month after summing the amount of months of the duration

\definecolor{color1}{HTML}{FFFFCC}
\definecolor{color2}{HTML}{FFEDA0}
\definecolor{color3}{HTML}{ff0000}
\definecolor{color4}{HTML}{00ff00}
\newcommand\Dganttbar[5]{
    \ganttbar[#5]{#1}{#3}{#4}\ganttbar[inline,bar label font=\tiny\bfseries, #5]{#2}{#3}{#4}
}
\begin{ganttchart}[
    expand chart=\textwidth,
    hgrid,
    vgrid,
    time slot format=isodate,
    time slot unit=month
]{2017-08-01}{2024-06-01}
    \gantttitlecalendar{year} \\
    \Dganttbar{(a)}{M}{2018-03-01}{2018-08-01}{bar/.append style={fill=color1}}
    \Dganttbar{(a)}{M}{2023-07-01}{2023-12-01}{bar/.append style={fill=color1}}
    \ganttvrule[]{$t$}{2018-02-01}
    \ganttvrule[]{$t'$}{2018-08-01}
    \ganttvrule[
    vrule label node/.append style={anchor=north west}
    ]{\hspace{-2pt} $\mathcal{T}_{t'}^s$}{2018-02-01}
    \ganttvrule[
    vrule label node/.append style={anchor=north west}
    ]{\hspace{50pt} $\mathcal{T}_t^m$}{2018-08-01}
    \ganttvrule[
    vrule label node/.append style={anchor=north west}
    ]{\hspace{50pt} $\mathcal{T}_t^M$}{2021-02-01}
    \ganttvrule[
    vrule label node/.append style={anchor=north west}
    ]{}{2023-08-01}
\end{ganttchart}


==> gantts/time_windows_init.tex <==
\definecolor{color1}{HTML}{FFFFCC}
\definecolor{color2}{HTML}{FFEDA0}
\definecolor{color3}{HTML}{ff0000}
\definecolor{color4}{HTML}{00ff00}
\newcommand\Dganttbar[5]{
    \ganttbar[#5]{#1}{#3}{#4}\ganttbar[inline,bar label font=\tiny\bfseries, #5]{#2}{#3}{#4}
}
\begin{ganttchart}[
    expand chart=\textwidth,
    hgrid,
    vgrid,
    time slot format=isodate,
    time slot unit=month
]{2017-08-01}{2024-06-01}
    % \gantttitlecalendar{year} \\
    \Dganttbar{(b)}{M}{2019-02-01}{2019-07-01}{bar/.append style={fill=color1}}
    \ganttvrule[
    vrule label node/.append style={anchor=north east}
    ]{\hspace{-40pt}$\mathcal{T}^{m_{ini}}_i$}{2018-05-01}
    \ganttvrule[
    vrule label node/.append style={anchor=north east}
    ]{\hspace{-80pt}$\mathcal{T}^{M_{ini}}_i$}{2020-01-01}
    % \ganttvrule[
    % vrule label node/.append style={anchor=north west}
    % ]{}{2020-02-01}
\end{ganttchart}


==> gantts/time_windows_mission.tex <==
\definecolor{color1}{HTML}{FFFFCC}
\definecolor{color2}{HTML}{FFEDA0}
\definecolor{color3}{HTML}{ff0000}
\definecolor{color4}{HTML}{00ff00}
\newcommand\Dganttbar[5]{
      \ganttbar[#5]{#1}{#3}{#4}\ganttbar[inline,bar label font=\tiny\bfseries, #5]{#2}{#3}{#4}
}
\begin{ganttchart}[
    expand chart=\textwidth,
    hgrid,
    vgrid,
    time slot format=isodate,
    time slot unit=month
]{2017-08-01}{2024-06-01}
    \gantttitlecalendar{year} \\
    \Dganttbar{(c)}{$j$}{2018-01-01}{2018-06-01}{bar/.append style={fill=color1}}
    \Dganttbar{(c)}{$j$}{2019-02-01}{2020-07-01}{bar/.append style={fill=color1}}
    % \Dganttbar{$i'$}{$j$}{2018-07-01}{2019-01-01}{bar/.append style={fill=color1}}
    \ganttvrule[]{$t$}{2017-12-01}
    \ganttvrule[
    vrule label node/.append style={anchor=north west}
    ]{\hspace{-2pt} $\mathcal{T}_{jt}^{MT}$}{2017-12-01}
    \ganttvrule[]{}{2018-06-01}
    \ganttvrule[]{$t'$}{2019-01-01}
    \ganttvrule[
    vrule label node/.append style={anchor=north west}
    ]{\hspace{-2pt} $\mathcal{T}_{jt'}^{MT}$}{2019-01-01}
    \ganttvrule[]{}{2019-07-01}
\end{ganttchart}


==> tables/clust1_20190408_remake.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
             case &  $t^{min}$ &  $t^{avg}$ &  non-zero &    vars &    cons &  no-int &  inf &  $g^{avg}$ \\
\midrule
             base &        2.2 &      222.0 &   51167.1 &  4310.7 &  6315.9 &       0 &    1 &        0.1 \\
      $| T |$=120 &       15.2 &      504.3 &   88668.3 &  5815.8 &  9161.6 &       0 &    6 &        1.8 \\
      $| J^P |$=2 &       21.9 &      899.4 &  101336.8 &  8350.3 & 12286.9 &       0 &    2 &        0.5 \\
      $| T |$=140 &       65.4 &     1446.9 &  115910.9 &  6738.7 & 11081.5 &       0 &    4 &        2.5 \\
 $\max \{rft\}$=1 &        5.4 &     2179.1 &   51167.1 &  4310.7 &  6315.9 &       0 &    1 &        1.7 \\
      $U^{min}$=5 &       17.0 &     2538.6 &   60950.1 &  5525.3 &  8583.6 &       0 &    3 &        3.9 \\
      $| J^P |$=3 &       65.7 &     2754.3 &  157213.7 & 12907.6 & 18915.8 &       3 &    8 &        2.0 \\
      $| J^P |$=4 &      178.1 &     3287.2 &  209747.2 & 17045.4 & 24947.4 &       3 &    9 &        2.6 \\
     $U^{min}$=20 &     3600.0 &     3600.0 &   53562.3 &  5379.8 &  8149.6 &      22 &    8 &        5.5 \\
     $U^{min}$=15 &     3600.0 &     3600.0 &   60716.4 &  5529.0 &  8573.6 &      10 &    6 &        6.7 \\
\bottomrule
\end{tabular}


==> tables/clust_params1_cplex.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
           case &  $t^{min}$ &  $t^{avg}$ &  non-zero &   vars &   cons &  no-int &  inf &  $g^{avg}$ \\
\midrule
   $H^{M}$=1200 &        1.5 &      219.5 &   40484.1 & 3654.6 & 5240.0 &       0 &    0 &        0.0 \\
   $HP^{K}$=0.3 &        2.9 &      404.4 &   44149.4 & 3862.8 & 5602.9 &       0 &    0 &        0.0 \\
     $E^{s}$=20 &        3.1 &      966.1 &   28830.4 & 3804.0 & 5051.6 &       0 &    4 &        0.0 \\
          $M$=4 &       10.1 &     1310.8 &   47463.2 & 4271.3 & 6249.7 &       0 &    2 &        0.2 \\
          $M$=8 &        9.9 &     1341.4 &   49399.6 & 4178.4 & 6022.8 &       0 &    3 &        0.4 \\
           base &        3.4 &     1354.0 &   47622.1 & 4143.0 & 6017.8 &       0 &    1 &        0.3 \\
 $C^{perc}$=0.2 &        3.4 &     1354.8 &   47622.1 & 4143.0 & 6017.8 &       0 &    1 &        0.2 \\
 $C^{perc}$=0.1 &       10.2 &     1504.9 &   48361.6 & 4231.9 & 6134.8 &       0 &    3 &        0.4 \\
     $E^{s}$=40 &       12.3 &     1524.0 &   63584.6 & 4492.7 & 6968.8 &       0 &    1 &        0.5 \\
     $E^{M}$=40 &       30.5 &     1897.6 &   68406.1 & 4534.6 & 7643.9 &       0 &    1 &        0.0 \\
     $E^{M}$=80 &       12.6 &     2573.7 &   27247.8 & 3826.1 & 4911.0 &       0 &    3 &        1.5 \\
   $HP^{K}$=0.7 &      158.5 &     2863.1 &   49381.6 & 4355.0 & 6221.8 &       0 &   41 &        1.0 \\
    $H^{M}$=800 &       85.1 &     3308.8 &   49906.1 & 4306.7 & 6262.7 &       0 &    5 &        2.6 \\
    $U^{min}$=5 &     1346.7 &     3490.1 &   59458.7 & 5493.7 & 8488.7 &       1 &    3 &        3.5 \\
   $U^{min}$=20 &     3600.0 &     3600.0 &   51789.8 & 5340.1 & 8031.3 &      20 &   11 &        5.4 \\
   $U^{min}$=15 &     3600.0 &     3600.0 &   59239.2 & 5500.9 & 8484.6 &      10 &    7 &        5.8 \\
\bottomrule
\end{tabular}


==> tables/clust_params1_cplex_cut_statistics.tex <==
\begin{tabular}{lrrrr}
\toprule
           case &  rinit &  rcuts &  icuts &    nodes \\
\midrule
           base &   16.0 &    2.3 &    9.7 & 201500.9 \\
     $E^{s}$=20 &    1.8 &    0.5 &    4.5 & 117454.8 \\
     $E^{s}$=40 &   17.7 &    3.4 &   28.7 & 184485.4 \\
          $M$=4 &   18.1 &    2.3 &   14.4 & 166611.8 \\
          $M$=8 &   12.4 &    2.1 &    5.9 & 165111.2 \\
     $E^{M}$=40 &   41.3 &    6.3 &   11.1 &  85931.6 \\
     $E^{M}$=80 &    4.1 &    1.8 &    9.8 & 240290.1 \\
   $H^{M}$=1200 &   17.1 &    0.7 &    1.3 &  27987.9 \\
    $H^{M}$=800 &   10.7 &    5.4 &   22.6 & 952219.4 \\
   $HP^{K}$=0.3 &   16.7 &    0.4 &    2.9 &  37805.5 \\
   $HP^{K}$=0.7 &   16.8 &    9.6 &   29.2 & 587426.3 \\
   $U^{min}$=15 &   32.3 &   16.0 &   11.2 &      NaN \\
   $U^{min}$=20 &   26.7 &    9.2 &   12.5 &      NaN \\
    $U^{min}$=5 &   21.4 &    7.1 &   25.0 & 352894.0 \\
 $C^{perc}$=0.1 &   16.2 &    2.7 &    3.8 &  69892.2 \\
 $C^{perc}$=0.2 &   15.9 &    2.2 &    9.7 & 173594.1 \\
\bottomrule
\end{tabular}


==> tables/clust_params1_cplex_v2.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
         case &  $t^{min}$ &  $t^{avg}$ &  non-zero &   vars &   cons &  no-int &  inf &  $g^{avg}$ \\
\midrule
 $HP^{K}$=0.3 &        1.8 &        5.2 &   50976.5 & 4275.5 & 6273.0 &       0 &    0 &        0.0 \\
 $H^{M}$=1200 &        2.1 &       76.7 &   51030.3 & 4295.0 & 6298.2 &       0 &    0 &        0.1 \\
   $E^{s}$=20 &        1.6 &      172.8 &   29772.8 & 3826.1 & 5120.3 &       0 &    3 &        0.2 \\
   $E^{s}$=40 &        4.0 &      266.8 &   64152.6 & 4496.1 & 6994.6 &       0 &    1 &        0.4 \\
         base &        2.2 &      310.6 &   51167.1 & 4310.7 & 6315.9 &       0 &    1 &        0.3 \\
   $E^{M}$=40 &        8.1 &      530.9 &   68612.7 & 4525.5 & 7632.9 &       0 &    0 &        0.2 \\
   $E^{M}$=80 &        1.5 &     1250.6 &   28257.9 & 3877.8 & 5010.4 &       0 &    3 &        1.9 \\
 $HP^{K}$=0.7 &       80.7 &     1746.9 &   50805.8 & 4393.9 & 6320.6 &       0 &   42 &        2.9 \\
  $H^{M}$=800 &        4.4 &     2168.5 &   51219.7 & 4327.2 & 6327.2 &       0 &    5 &        2.7 \\
  $U^{min}$=5 &       24.6 &     2650.3 &   60950.1 & 5525.3 & 8583.6 &       0 &    3 &        4.3 \\
 $U^{min}$=20 &     3600.0 &     3600.0 &   53562.3 & 5379.8 & 8149.6 &      25 &    8 &        5.2 \\
 $U^{min}$=15 &     3600.0 &     3600.0 &   60716.4 & 5529.0 & 8573.6 &      10 &    6 &        6.3 \\
\bottomrule
\end{tabular}


==> tables/clust_params2_cplex.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
             case &  $t^{min}$ &  $t^{avg}$ &  non-zero &    vars &    cons &  no-int &  inf &  $g^{avg}$ \\
\midrule
             base &        3.4 &     1354.7 &   47622.1 &  4143.0 &  6017.8 &       0 &    1 &        0.3 \\
      $| T |$=120 &       41.5 &     2271.1 &   86927.5 &  5798.7 &  9089.7 &       0 &    6 &        0.2 \\
 $\max \{rft\}$=1 &       22.6 &     2935.7 &   49838.5 &  4288.8 &  6249.8 &       0 &    1 &        1.7 \\
      $| T |$=140 &      116.7 &     3343.7 &  114014.5 &  6709.8 & 10991.6 &       0 &    4 &        2.2 \\
      $| J^P |$=2 &      120.5 &     3349.9 &   98906.0 &  8252.6 & 12112.7 &       0 &    5 &        0.8 \\
      $| J^P |$=3 &     3600.0 &     3600.0 &  152865.3 & 12828.6 & 18690.3 &       1 &    8 &        2.1 \\
      $| J^P |$=4 &     3600.0 &     3600.0 &  204013.2 & 16948.7 & 24662.4 &       2 &    9 &        2.6 \\
\bottomrule
\end{tabular}


==> tables/clust_params2_cplex_cut_statistics.tex <==
\begin{tabular}{lrrrr}
\toprule
             case &  rinit &  rcuts &  icuts &    nodes \\
\midrule
             base &   16.0 &    2.3 &    9.7 & 173594.1 \\
      $| J^P |$=2 &   15.3 &    3.3 &   32.3 &  45273.0 \\
      $| J^P |$=3 &   16.0 &    4.6 &   40.5 &      NaN \\
      $| J^P |$=4 &   15.5 &    5.0 &   41.2 &      NaN \\
      $| T |$=120 &   24.8 &   14.0 &   24.4 & 174785.9 \\
      $| T |$=140 &   22.6 &   19.0 &   38.6 & 111043.3 \\
 $\max \{rft\}$=1 &    9.4 &    3.7 &   62.0 & 127605.8 \\
\bottomrule
\end{tabular}


==> tables/cut_comparison.tex <==
\begin{tabular}{lrrrr}
\toprule
            Type of cut &  base &  $U^{min}$=5 &  $U^{min}$15 &  $U^{min}$=20 \\
\midrule
                 Clique &     5 &      9 &      11 &      30 \\
                  Cover &    16 &     17 &      14 &      11 \\
                   Flow &     9 &    315 &     219 &     166 \\
              GUB cover &     3 &      3 &       3 &       5 \\
      Gomory fractional &    28 &    222 &     306 &     228 \\
          Implied bound &    96 &    102 &      96 &     354 \\
       Lift and project &    15 &     48 &      66 &      40 \\
 Mixed integer rounding &    57 &    398 &     412 &     386 \\
              Zero-half &    36 &     65 &      47 &      36 \\
\bottomrule
\end{tabular}


==> tables/heuristic_comp.tex <==
\begin{tabular}{lrrrr}
\toprule
             case &  $t^{avg}_H$ &  $t^{avg}_M$ &  $\%Init_H$ &  $g^{avg}_{HM}$ \\
\midrule
             base &         23.7 &        247.1 &       100.0 &            22.0 \\
      $U^{min}$=5 &         92.8 &       2417.5 &       100.0 &            19.0 \\
      $| J^P |$=2 &         86.2 &        706.9 &       100.0 &            22.0 \\
      $| J^P |$=3 &        217.1 &       1979.5 &       100.0 &            23.0 \\
      $| J^P |$=4 &        401.1 &       3102.1 &       100.0 &            19.5 \\
      $| T |$=120 &         47.8 &        247.6 &       100.0 &            19.7 \\
      $| T |$=140 &         65.8 &       1493.3 &       100.0 &            23.4 \\
 $\max \{rft\}$=1 &         23.7 &       2214.1 &       100.0 &            89.9 \\
\bottomrule
\end{tabular}

